Integrability of two-species partially asymmetric exclusion processes

We work towards the classification of all one-dimensional exclusion processes with two species of particles that can be solved by a nested coordinate Bethe Ansatz. Using the Yang-Baxter equations, we obtain conditions on the model parameters that ensure that the underlying system is integrable. Three classes of integrable models are thus found. Of these, two classes are well known in literature, but the third has not been studied until recently, and never in the context of the Bethe ansatz. The Bethe equations are derived for the latter model as well as for the associated dynamics encoding the large deviation of the currents.

==> removed.tex <==
%   DESCRIPTION OF COLLISION EQUATIONS
Note that in its literal interpretation, \eref{evproblem} is only valid for configurations in which no two particles are on adjacent sites.
We may allow it to hold in all configurations if we fix the amplitudes so that they satisfy so-called collision equations.
These equations ensure that when two particles are on adjacent sites, the amplitudes corresponding to forbidden processes cancel (in the $11$ and $22$ cases), or are replaced exactly by the rates corresponding to overtaking processes (in the $12$ and $21$ cases).
Note that the overtaking rates are not included in \eref{evproblem} {\it a priori}.
Focusing on pairs of permutations that differ by only one pair of adjacent indices, the collision equations read
\numparts
\begin{eqnarray}
    \fl -(\alpha + x/\alpha ) 
    (A^{11}_{ij} z_j + A^{  11  }_{  ji   } z_i)
    +  (A^{  11  }_{  ij   } + A^{  11  }_{  ji   })
    + x  z_i z_j (A^{  11  }_{  ij   } + A^{  11  }_{  ji   }) = 0 \;, \label{coll_nested_a}
    \\ \fl 
    -(1+x) 
    (A^{  22  }_{  ij   } z_j + A^{  22  }_{  ji   } z_i)
    + (A^{  22  }_{  ij   } + A^{  22  }_{  ji   })
    + x  z_i z_j (A^{  22  }_{  ij   } + A^{  22  }_{  ji   }) = 0 \;, \label{coll_nested_b}
    \\ \fl
    -(\alpha + x ) 
    (A^{  12  }_{  ij   } z_j + A^{  12  }_{  ji   } z_i)
    + (A^{  12  }_{  ij   } + A^{  12  }_{  ji   })
    + x  z_i z_j (A^{  12  }_{  ij   } + A^{  12  }_{  ji   }) = 
    \nonumber \\ 
    -\beta _+
    (A^{  12  }_{  ij   } z_j + A^{  12  }_{  ji   } z_i)
    + \alpha \beta _-
    (A^{  21  }_{  ij   } z_j + A^{  21  }_{  ji   } z_i) \;, \label{coll_nested_c}
    \\ \fl
    -(1 + x/\alpha ) 
    (A^{  21  }_{  ij   } z_j + A^{  21  }_{  ji   } z_i)
    + (A^{  21  }_{  ij   } + A^{  21  }_{  ji   })
    + x  z_i z_j (A^{  21  }_{  ij   } + A^{  21  }_{  ji   }) = 
    \nonumber \\  
    -\beta _-
    (A^{  21  }_{  ij   } z_j + A^{  21  }_{  ji   } z_i)
    + \beta _+/\alpha 
    (A^{  12  }_{  ij   } z_j + A^{  12  }_{  ji   } z_i) \;. \label{coll_nested_d}
\end{eqnarray}

% DERIVATION OF BEQ FOR SOLUTION 3
Before we proceed to derive the Bethe equations, we reformulate the problem slightly, in order to make it more conducive to calculating current statistics.

Firstly, we define the joint probability of seeing the system in configuration $\cal C$ and the total displacement of all second class particles being $Y$ at a time $t$ as $P_t({\cal C},Y)$.
Its generating function with auxiliary variable $\gamma $ is given by
\begin{equation}
    F_t({\cal C},\gamma ) = \sum\limits_{Y = -\infty}^{\infty} \rme ^{\gamma Y}P_t({\cal C},Y) \;.
\end{equation}
Note that this is closely related to the moment generating function of $Y$ at time $t$,
\begin{equation}
    \langle \rme ^{\gamma Y_t}\rangle = \sum\limits_{\cal C} F_t({\cal C},\gamma )\;.
\end{equation}
To obtain the evolution equation for $F_t ({\cal C},\gamma )$, it is convenient to split the Markov operator in \eref{master} into components
\begin{equation}
    {\cal M} = {\cal M}_0 + {\cal M}_{1,+1} + {\cal M}_{1,-1} + {\cal M}_{2,+1} + {\cal M}_{2,-1}\;,
\end{equation}
where ${\cal M}_0$ contains the diagonal elements (defined such that all columns add to 0), and ${\cal M}_{\mu ,\pm 1}$ contains the rates of processes in which a particle of species $\mu $ hops to the right $(+1)$ or left $(-1)$.
Processes in which the defect overtakes second class particles are counted as hops of the defect and are thus included in ${\cal M}_{1,\pm 1}$.
Then the evolution equation for $F_t ({\cal C},\gamma )$ is given by
\begin{equation}
    \frac{\partial F_t ({\cal C},\gamma )}{\partial t} = 
    \sum\limits_{{\cal C}'} {\cal M}_\gamma ({\cal C},{\cal C}') F_t({\cal C}',\gamma ) \;,
\end{equation}
where ${\cal M} _\gamma $ is the deformed Markov operator
\begin{equation}
    {\cal M} _\gamma = {\cal M}_0 + {\cal M}_{1,+1} + {\cal M}_{1,-1} + \rme ^\gamma {\cal M}_{2,+1} + \rme ^{-\gamma }{\cal M}_{2,-1}\;.
\end{equation}

We now use a modified coordinate Bethe ansatz to solve the eigenvalue-eigenvector problem for ${\cal M} \gamma $.
We could use an ansatz similar to \eref{ansatz} and collision equations \eref{coll_nested_a}-\eref{coll_nested_d} to derive the Bethe equations.
However, as there is only one defect, we do not need to make use of the full nested ansatz.
Instead, it is simpler to fix the labelling such that the defect is always particle number 1, which can be done without loss of generality due to the translational invariance of the system.
Then the eigenvalue-eigenvector problem can be written as
\begin{eqnarray}
    \fl \lambda (\gamma )\psi (x_1 ,\dots ,x_M) = 
    -[M_2(p+q) + \alpha p+q/\alpha ]\psi (x_1 ,\dots ,x_M) \nonumber \\
    + \alpha p \psi (x_1 -1,\dots ) + q/\alpha \psi (x_1 +1,\dots ) \nonumber \\
    + \sum\limits _{j=2}^{M} [p\rme ^\gamma \psi (\dots , x_j -1,\dots ) 
    + q \rme ^{-\gamma }\psi (\dots , x_j + 1,\dots )] \;,
\end{eqnarray}
and the ansatz takes the simpler form
\begin{equation}
    \psi (x_1, \dots ,x_M) =
    \alpha ^{x_1} \rme ^{-\gamma x_1} \sum\limits _\sigma A_\sigma
    z_{\sigma (1)}^{x_1} \dots  z_{\sigma (M)}^{x_M} \;,
    \label{ansatz2}
\end{equation}
which gives for the eigenvalues of the deformed Markov operator,
\begin{equation}
    \lambda (\gamma )= -[M_2(p+q) + \alpha p+q/\alpha ] 
    + \sum\limits_{j=1}^{M}(p\rme^\gamma z_j ^{-1} + q\rme ^{-\gamma} z_j )\;.
    \label{evalue}
\end{equation}
We remark that although the derivation so far has been general, we are particularly interested in the eigenvalue with the largest real part.
It has the property $\lambda (\gamma )\to 0 $ as $\gamma \to 0$.
That such an eigenvalue exists and is unique follows from the Perron-Frobenius theorem and the fact that the (undeformed) Markov operator ${\cal M}$ is a transition rate matrix.
In the limit $t\to \infty $, this eigenvalue will dominate the dynamics and will govern the statistics of $Y_t$.


%% Introducing ansatz, p1q1=p2q2 condition

If we impose the condition
\begin{equation}
    p_1q_1=p_2q_2\;, \label{pqpq}
\end{equation}
we can set
\begin{equation}
    p_1 = \alpha p_2\;,\qquad q_1=q_2/\alpha \;, \label{alpha}
\end{equation}
for some constant $\alpha $.
It is also convenient to define the following dimensionless parameters
\begin{eqnarray}
    x=q_2/p_2 \;,\\
   \beta_{12}=b_{12}/p_2 \;,\qquad \beta_{21}=b_{21}/p_2 \;.
\end{eqnarray}
In this case, the problem is diagonalized by the following modified nested coordinate BA
\begin{equation}
    \psi ^{Q_1, \dots ,Q_M} (x_1, \dots ,x_M) =
    r_{Q_1} ^{x_1} \dots r_{Q_M} ^{x_M} \sum\limits _\sigma A^{Q_1, \dots ,Q_M}_\sigma
    z_{\sigma (1)}^{x_1} \dots  z_{\sigma (M)}^{x_M} \;,
    \label{ansatz}
\end{equation}
where
\begin{equation}
    r_1 = \alpha \;,\qquad r_2 =1\;,\label{r1r2}
\end{equation}
$\sigma $ indicates the permutations of the integers $1, \dots ,M$; and the $A$'s and $z$'s are undetermined complex amplitudes and Bethe roots respectively.
A similar modification of the standard coordinate BA was introduced in \cite{derrida1999bethe}, although there it was used only for a totally asymmetric problem with one defect particle.

%% Abstract
We consider a broad class of one-dimensional exclusion processes on a ring with two species of particles and overtaking. We investigate their
 solution by a nested coordinate Bethe ansatz.
The deformed time-evolution problem for these models, 
relevant for calculating large deviation functions of currents, is also considered.
The Yang-Baxter equations for the ansatz are derived and are used to obtain conditions on the model parameters that ensure that the underlying models are integrable.
Three classes of integrable models are found.
Of these, two classes are well known in literature, but the third has not been studied until recently, and never in the context of the Bethe ansatz.
The Bethe equations for the new model are then derived.
{\mre I am happy for  Kirone's paragraph to replace the previous paragraph}

%% Discussion of p1q1=p2q2
{\mre This paragraph to be refined}
It remains somewhat unclear whether \eref{pqpq} is a necessary requirement for integrability.
Here, it appears simply because \eref{ansatz} is the most general known coordinate ansatz and it requires \eref{pqpq} to work.
However, we remark that using an algebraic approach, a similar condition was derived from the YBE of the $15$-vertex model \cite{vieira2021solutions}.
With certain choices of parameters, the $15$-vertex model can be mapped to a two-species PASEP with overtaking.
This suggests that \eref{ansatz} is indeed the most general coordinate ansatz for the two-species problem.

Old equation (21)

\begin{eqnarray}
   \Phi_{ij} = [{\cal D}_{ij}^2-{\cal D}_{ij}(\kappa _1+\kappa _2)z_i - \beta_{12} \beta_{21} z_i^2]^{-1}\;.
\end{eqnarray}

Old paragraph describing $\alpha=1$ chain:

The choices $x=0$ and $\alpha=1$ are sufficient to satisfy the YBE fully for the 112 and 122 blocks, giving solutions 1 and 2 respectively.

